Time-Sliced Quantum Circuit Partitioning for Modular Architectures

Current quantum computer designs will not scale. To scale beyond small prototypes, quantum architectures will likely adopt a modular approach with clusters of tightly connected quantum bits and sparser connections between clusters. We exploit this clustering and the statically-known control flow of quantum programs to create tractable partitioning heuristics which map quantum circuits to modular physical machines one time slice at a time. Specifically, we create optimized mappings for each time slice, accounting for the cost to move data from the previous time slice and using a tunable lookahead scheme to reduce the cost to move to future time slices. We compare our approach to a traditional statically-mapped, owner-computes model. Our results show strict improvement over the static mapping baseline. We reduce the non-local communication overhead by 89.8\% in the best case and by 60.9\% on average. Our techniques, unlike many exact solver methods, are computationally tractable.

==> text/motivation.tex <==
%\vspace{0.7cm}
\section{\reviewaddition{Motivation}} \label{sec:motivation}

\reviewaddition{Current quantum hardware, which has on the order of tens of physical qubits, is insufficient to run important quantum algorithms. Scaling these devices even to a moderate size with low error rates has proven extremely challenging. Manufacturers of quantum hardware such as IBM and IonQ have had only limited success in extending the number of physical qubits present on a single contiguous piece of hardware. Issues on these devices such as crosstalk error scaling with the number of qubits or increased difficulty in control will limit the size this single-chip architecture can achieve \cite{bruzewicz2019trapped, brown2016co}}. 

\reviewaddition{Due to these challenges, as well as developing technology for communicating between different quantum chips \cite{blakestad2009high, wallraff2018deterministic}, we expect quantum hardware to scale via a modular approach similar to how a classical computer could be scaled increasing the number of processors not just the size of the processors. Two of the leading quantum technologies, ion trap and superconducting physical qubits, are already beginning to explore this avenue and experimentalists project modularity will be the key to moving forward \cite{brecht2016multilayer, devoret2013superconducting, duan2010colloquium, bapat2018unitary, maslov2018outlook, monroe2013scaling, hucul2017spectroscopy}. Technology such as resonant busses in superconducting hardware or optical communication techniques in ion trap devices will enable this more distributed approach to quantum computing, having many smaller, well-connected devices with sparser and more expensive non-local connections between them. Optimistically, due to current technology in the near term, we expect these non-local communication operations to be somewhere between 5-100x higher latency than in-cluster communication.}

\reviewaddition{With cluster-based approaches becoming more prominent, new compiler techniques for mapping and scheduling of quantum programs are needed. Furthermore, as the size of executable computations increase it becomes more and more critical to employ program mappings that exhibit both the adaptivity of dynamic techniques and the global optimization of static techniques.  Key to realizing both advantages is to simplify the problem.  Since non-local communication is dominant, we can focus on only non-local costs.  This simplification, along with static knowledge of all control flow, allows us to map a program in many timeslices with substantial lookahead for future program behavior.  This approach would not be computationally tractable on a non-clustered machine.}  

